Symbolic Representation for Any-to-Any Generative Tasks

We propose a symbolic generative task description language and a corresponding inference engine capable of representing arbitrary multimodal tasks as structured symbolic flows. Unlike conventional generative models that rely on large-scale training and implicit neural representations to learn cross-modal mappings, often at high computational cost and with limited flexibility, our framework introduces an explicit symbolic representation comprising three core primitives: functions, parameters, and topological logic. Leveraging a pre-trained language model, our inference engine maps natural language instructions directly to symbolic workflows in a training-free manner. Our framework successfully performs over 12 diverse multimodal generative tasks, demonstrating strong performance and flexibility without the need for task-specific tuning. Experiments show that our method not only matches or outperforms existing state-of-the-art unified models in content quality, but also offers greater efficiency, editability, and interruptibility. We believe that symbolic task representations provide a cost-effective and extensible foundation for advancing the capabilities of generative AI.

==> figures/task_with_image.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{figures/fig_task_with_image.pdf}
    \caption{
\textbf{Qualitative results of image manipulation and generation.}
% 
Starting from input image(s), the tasks include local image editing, image fusion, image completion, viewpoint synthesis, 3D mesh creation, and animation. Each example shows both the input image(s) and simplified task description in natural language.
}
    \label{fig:task_with_image}
\end{figure*}

==> figures/task_with_text.tex <==
\begin{figure*}[h]
    \centering
\includegraphics[width=\textwidth]{figures/fig_task_with_text.pdf}
    \caption{
\textbf{Examples of text-driven multimodal generation tasks.} Starting from natural language descriptions, the tasks include text-to-image creation, text-guided image fusion, text-to-video animation, text-to-audio conversion, and text-to-3D mesh modeling. Each example shows both the text instruction and the generated output in different modalities.
    }
    \label{fig:task_with_text}
\end{figure*}

==> tables/alignment_rank_comparison.tex <==
% author: yifei

\begin{table*}[th]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Alignment rank comparison} across unified multi-modal frameworks.}
\label{tab:alignment_rank_comparison}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccccccccccc}
\hline
\toprule
\textbf{Method} & \textbf{Inpainting} & \textbf{Img merge} & \textbf{Outpainting} & \textbf{NVS} & \textbf{Merge model} & \textbf{I-2-3D}  & \textbf{Multi-view img} & \textbf{I2V} & \textbf{Text2Audio} & \textbf{T2I} & \textbf{Text2Mesh} & \textbf{T2V} \\
\midrule
% x：模型不具备该任务能力
% y：缺失该任务的系列实验数据 -> 1
% z：缺失该模型的系列实验数据
Gen-3~\cite{runway2024gen3} & x    & x   & x   & 1 & 1 & 1 & 1 & 1.07 & x & x    & 1 & 1 \\
Show-o~\cite{xie2024showo} & 1.69 & x   & 1.4 & 1 & 1 & 1 & 1 & x    & x & 2.78 & 1 & 1 \\
SEED-X~\cite{ge2024seed} & x    & 1.2 & x   & 1 & 1 & 1 & 1 & x    & x & 2    & 1 & 1 \\
LWM~\cite{liu2023world} & x    & x   & x   & 1 & 1 & 1 & 1 & x    & x & 4.08 & 1 & 1 \\
Unified-IO 2~\cite{lu2023unifiedio2scalingautoregressive} & z    & z   & z   & 1 & 1 & 1 & 1 & z    & 2 & 4.62 & 1 & 1 \\
Ours & 1.31 & 1.8 & 1.6 & 1 & 1 & 1 & 1 & 1.93 & 1 & 1.52 & 1 & 1 \\
\bottomrule

\end{tabular}%
% }
\end{table*}

==> tables/full_results.tex <==
\begin{table*}[th]
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1.1}
    \caption{\textbf{Performance comparison on syntax style.} We report the pass rate for a single run (Pass@1/\%). ``Comp'' denotes ``Compile'', ``Exec'' denotes ``Execute''.}
    \label{tab:benchmark_evaluation}
    \centering
    \begin{tabular}{ccccccccccccccccccccccccc}
        \hline

        \hline
        \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Syntax}}}& \multicolumn{2}{c}{\textbf{Inpainting}} & \multicolumn{2}{c}{\textbf{Img merge}} & \multicolumn{2}{c}{\textbf{Outpainting}} & \multicolumn{2}{c}{\textbf{Novel view syn.}}& \multicolumn{2}{c}{\textbf{Merge model}}& \multicolumn{2}{c}{\textbf{Img2Mesh}}\\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} &
        & Comp & Exec & Comp & Exec & Comp & Exec & Comp & Exec & Comp & Exec & Comp & Exec \\
        \midrule
        % GenAgent~\cite{xue2024genagent}  & $0.7$ & $0.3$ & $0.7$ & $0.2$ & \textbf{1.0} & \textbf{0.9} & $0.5$ & $0.2$ & $0.6$ & $0.3$  & $0.9$ & $0.9$\\
        \multicolumn{2}{l}{Dataflow~\cite{xue2024genagent,gupta2023visual}}  & $\textbf{1.0}$ & $\textbf{0.9}$ & $\textbf{1.0}$ & $0.7$ & $0.9$ & $0.9$ & $0.7$ & $0.5$ & $\textbf{1.0}$ & $\textbf{0.9}$ & $\textbf{1.0}$ & $\textbf{1.0}$ \\
        \multicolumn{2}{l}{Pseudo-natural} & $0.9$ & $\textbf{0.9}$ & $0.9$ & $\textbf{0.8}$ &$0.9$ & $0.9$ & $0.8$ & $0.7$ & $0.9$ & $\textbf{0.9}$ & $0.8$ & $0.7$ \\
        \rowcolor[gray]{.9} 
        \multicolumn{2}{l}{Declarative} & $\textbf{1.0}$ & $0.7$ & $0.9$ & $0.7$ & $\textbf{1.0}$ & $\textbf{1.0}$ & $\textbf{0.9}$ & $\textbf{0.8}$ & $0.9$ & $\textbf{0.9}$ & $\textbf{1.0}$ & $0.8$ \\
        \midrule
        \multicolumn{2}{c}{\textbf{Multi-view img}} & \multicolumn{2}{c}{\textbf{Img2Video}}& \multicolumn{2}{c}{\textbf{Text2Audio}}& \multicolumn{2}{c}{\textbf{Text2Img}}& \multicolumn{2}{c}{\textbf{Text2Mesh}}& \multicolumn{2}{c}{\textbf{Text2Video}}& \multicolumn{2}{c}{\textbf{Average}} \\
                \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} 
        Comp & Exec & Comp & Exec & Comp & Exec & Comp & Exec & Comp & Exec & Comp & Exec & Comp & Exec \\
        \midrule
        % GenAgent~\cite{xue2024genagent} & $0.8$ & $0.0$ & \textbf{1.0} & \textbf{0.9}  &$0.8$ &$0.4$ &\textbf{1.0} & $0.7$ & $0.8$
        % & $0.6$ & $0.7$ &\textbf{0.1}\\ 
         $0.8$ & $0.1$ & $\textbf{1.0}$ & $0.9$ & $0.6$ & $0.4$ &$\textbf{1.0}$ &$0.9$ & $0.3$ & $0.3$ & $\textbf{1.0}$ & $\textbf{1.0}$ & $0.86$ & $0.71$ \\

        $0.9$ & $0.4$ & $\textbf{1.0}$ & $\textbf{1.0}$ & $0.6$ & $0.4$ & $0.8$ & $0.8$ & $0.3$ & $0.0$ & $0.9$ & $0.8$ & $0.81$ & $0.63$\\
        \rowcolor[gray]{.9} 
       $\textbf{1.0}$ & $\textbf{1.0}$ & $\textbf{1.0}$ & $\textbf{1.0}$ & $\textbf{1.0}$ & $\textbf{0.8}$ & $\textbf{1.0}$ & $\textbf{1.0}$ & $\textbf{1.0}$ & $\textbf{0.8}$ & $\textbf{1.0}$ & $0.9$ & $\textbf{0.98}$ & $\textbf{0.87}$\\
        \hline

        \hline
    \end{tabular}
\end{table*}

==> tables/function_comparison.tex <==
\begin{table}[th]
\centering
\scriptsize
\setlength{\tabcolsep}{0.7pt}
\caption{\textbf{Capability comparison} across unified multi-modal frameworks.}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccccccc}
\hline
\toprule
\textbf{Method} & \textbf{Inpaint} & \textbf{Img merg} & \textbf{Outpaint} & \textbf{NVS} & \textbf{Merge model} & \textbf{I2Mesh}  \\
\midrule
Gen-3~\cite{runway2024gen3} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
Show-o~\cite{xie2024showo} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} & \ding{55} \\
SEED-X~\cite{ge2024seed} & \ding{55} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
LWM~\cite{liu2023world} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
Unified-IO 2~\cite{lu2023unifiedio2scalingautoregressive} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{51}\\
Ours & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
% \bottomrule
\toprule
\textbf{Method} & \textbf{MultiView} & \textbf{I2V} & \textbf{T2A} & \textbf{T2I} & \textbf{T2Mesh} & \textbf{T2V} \\
\midrule
Gen-3~\cite{runway2024gen3} & \ding{55} & \ding{51} & \ding{55} & \ding{55}  & \ding{55} & \ding{51} \\
Show-o~\cite{xie2024showo} & \ding{55} & \ding{55} & \ding{55} & \ding{51}  & \ding{55} & \ding{55} \\
SEED-X~\cite{ge2024seed} & \ding{55} & \ding{55} & \ding{55} & \ding{51}  & \ding{55} & \ding{55} \\
LWM~\cite{liu2023world} & \ding{55} & \ding{55} & \ding{55} & \ding{51}  & \ding{55} & \ding{55} \\
Unified-IO 2~\cite{lu2023unifiedio2scalingautoregressive} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{51}\\
Ours & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
\bottomrule
\hline
\end{tabular}%
% }
\end{table}

==> tables/main_results.tex <==
\begin{table}[th]
\centering
% \scriptsize
\setlength{\tabcolsep}{4.5pt}
    \caption{\textbf{Performance on the Uni-Gen benchmark.} We report the pass rate for a single run (Pass@1) and the pass rate for five runs (Pass@5).}
    \label{tab:benchmark_evaluation}
    \centering
    \begin{tabular}{lcccc}
        \hline

        \hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Pass@1} (\%)} & \multicolumn{2}{c}{\textbf{Pass@5} (\%)} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & \textbf{Compile} & \textbf{Execute} & \textbf{Compile} & \textbf{Execute} \\
        \midrule
        % VisualProg~\cite{gupta2023visual} \\
        % Unified-IO~\cite{lu2022unified} \\
        % Painter~\cite{wang2022image} \\
        GenAgent~\cite{xue2024genagent}  & $0.79$ & $0.46$ & & \\
        Ours &  $0.84$ & $0.63$ & & \\
        $Ours_{newcode}$ &\textbf{0.97} & \textbf{0.77} & &\\
        \hline

        \hline
    \end{tabular}
\end{table}



==> tables/quality_rank_comparison.tex <==
% author: yifei

\begin{table*}[th]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Quality rank comparison} across unified multi-modal frameworks.}
\label{tab:quality_rank_comparison}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccccccccccc}
\hline
\toprule
\textbf{Method} & \textbf{Inpainting} & \textbf{Img merge} & \textbf{Outpainting} & \textbf{NVS} & \textbf{Merge model} & \textbf{I-2-3D}  & \textbf{Multi-view img} & \textbf{I2V} & \textbf{Text2Audio} & \textbf{T2I} & \textbf{Text2Mesh} & \textbf{T2V} \\
\midrule
% x：模型不具备该任务能力
% y：缺失该任务的系列实验数据
% z：缺失该模型的系列实验数据
Gen-3~\cite{runway2024gen3} & x    & x   & x    & y & y & y & y & 1.03 & x    & x    & y & y \\
Show-o~\cite{xie2024showo} & 1.56 & x   & 1.42 & y & y & y & y & x    & x    & 2.9  & y & y \\
SEED-X~\cite{ge2024seed} & x    & 1.2 & x    & y & y & y & y & x    & x    & 2    & y & y \\
LWM~\cite{liu2023world} & x    & x   & x    & y & y & y & y & x    & x    & 4.38 & y & y \\
Unified-IO 2~\cite{lu2023unifiedio2scalingautoregressive} & z    & z   & z    & y & y & y & y & z    & 1.98 & 4.3  & y & y \\
Ours & 1.44 & 1.8 & 1.58 & 1 & 1 & 1 & 1 & 1.97 & 1.02 & 1.42 & 1 & 1 \\
\bottomrule

\end{tabular}%
% }

\end{table*}
